Commuting time geometry of ergodic Markov chains

We show how to map the states of an ergodic Markov chain to Euclidean space so that the squared distance between states is the expected commuting time. We find a minimax characterization of commuting times, and from this we get monotonicity of commuting times with respect to equilibrium transition rates. All of these results are familiar in the case of time-reversible chains, where techniques of classical electrical theory apply. In presenting these results, we take the opportunity to develop Markov chain theory in a `conformally correct' way

==> commute_dot_bib <==
\input{bibstrings}
@String(CACM="Communications of the ACM")
@String(JACM="Journal of the ACM")
@String(IPL="Information Processing Letters")
@String(JCSS="Journal of Computer and System Sciences")
@String(tcs="Theoretical Computer Science")
@String(MST="Mathematical Systems Theory")
@String(IEEETC="IEEE Trans. Computers")
@String(IRETC="IRE Trans. Elect. Computers")
@String(IBMJR="IBM Journal of Research and Development")
@String(IBMJST="IBM J. Syst. and Tech.")
@String(SIAMJC="SIAM Journal on Computing")
@String(INFCONT="Information and Control")
@String(INFCOMP="Information and Computation")

@book{kelly:paint,
author={F. Kelly},
title={Reversibility and Stochastic Networks},
publisher={Wiley},
year={1979}
}

@article{kingman:paint,
author={J. F. C. Kingman},
title={Markov population processes},
journal={J. Appl. Prob.},
year={1969},
volume={6},
pages={1-18}
}


@misc{doyleSteiner:hideandseek,
author={Peter G. Doyle and Jean Steiner},
title={Hide and seek on surfaces and {M}arkov chains}
}

@misc{doylereeds:kneejerk,
title={The knee-jerk mapping},
author={Peter G. Doyle and Jim Reeds},
eprint={arXiv:math/0606068v1 [math.PR]}
}

@misc{doyle:seek,
title={The {K}emeny constant of a {M}arkov chain},
author={Peter G. Doyle},
eprint={arXiv:0909.2636v1 [math.PR]}
}


@article(cdrs:cat,
 author={D. Coppersmith and P. Doyle and P. Raghavan and M.
Snir},
 title={Random walks on weighted graphs, and applications to
on-line algorithms},
 journal=JACM,
 year=1993,
 volume=40,
 pages={454--476})

@book(doyleSnell:walks,
 author={Peter G. Doyle and J. Laurie Snell},
 title={Random Walks and Electric Networks},
 publisher={The Mathematical Association of America},
 year={1984},
 eprint={arXiv:math/0001057v1 [math.PR]}
)

@inproceedings(crrst:commute,
 author={Chandra, A. K. and Raghavan, P. and Ruzzo,
W.L. and Smolensky, R. and Tiwari, P.},
 title={The Electrical Resistance of a Graph
Captures its Commute and Cover Times},
 booktitle={Proceedings of the 21st Annual ACM
Symposium on Theory of Computing},
 year={1989},
 pages={574-586},
 month=may,
 address={Seattle})

@book{grinsteadSnell:prob,
 author={Charles M. Grinstead and J. Laurie Snell},
 title={Introduction to Probability},
 publisher={The American Mathematical Society},
 year={1997}
}

